Safe, Occlusion-Aware Manipulation for Online Object Reconstruction in Confined Spaces

Recent work in robotic manipulation focuses on object retrieval in cluttered spaces under occlusion. Nevertheless, the majority of efforts lack an analysis of conditions for the completeness of the approaches or the methods apply only when objects can be removed from the workspace. This work formulates the general, occlusion-aware manipulation task, and focuses on safe object reconstruction in a confined space with in-place rearrangement. It proposes a framework that ensures safety with completeness guarantees. Furthermore, an algorithm, which is an instantiation of this abstract framework for monotone instances is developed and evaluated empirically by comparing against a random and a greedy baseline on randomly generated experiments in simulation. Even for cluttered scenes with realistic objects, the proposed algorithm significantly outperforms the baselines and maintains a high success rate across experimental conditions.

==> 01-prev-introduction.tex <==
* Brief problem description: To reconstruct unknown objects online in a confined space and fully reveal the scene. 

* Why is it important? Reconstructing object models on the fly is a critical functionality for performing manipulation in unstructured setups, such as logistics and home environments. There are many manipulation tasks that can benefit from this functionality when the object models are unknown. For instance, object retrieval in clutter or rearranging objects to a specified placement (e.g., setting up a dinner table) may require to reconstruct at least some of the objects in the scene so as to perform safe and effective manipulation. This work focuses on the case that all of the objects need to be reconstructed in order to safely address a problem so as to understand the requirements for achieving completeness guarantees in this domain. 

* Why is it challenging? 
you need a paragraph explaining why it is difficult

* What has been done and what has not been unaddressed?
relatively new area - because a lot of work assumed known object models
most of the work without knowing object models does not provide any guarantees  in terms of safety and completeness (learning-based - which is desirable for efficiency but it would be great if ML was used in the context of safe framework to improve efficiency)

* what are the contributions of this work? For each one you may want to expand upon and say why each point is novel and important. 


% \begin{enumerate}
% \item Background
% \item Existing work on the topic. Their limitations. Major limitations in the literature
% \item Key observation that leads to this paper
% \item summary of contributions and approach
% \end{enumerate}
Robotic manipulation has wide applications in manufacturing, logistics and domestic domains. Recent efforts have focused on enabling effective robot operation in unstructured environments, which requires robust algorithmic and software design. One such effort involves interactive perception, which incorporates perception into Task and Motion Planning (TAMP) so that they complement each other to solve sophisticated tasks \cite{bohg2017interactive}. This relates to the problem of retrieving objects in clutter \cite{bejjani2021occlusion,van2014probabilistic} and reconstructing object models \cite{huang2019building}.

Approaches for such tasks can be critical when visibility of the scene is limited. For instance, consider a logistic setup where a robot manipulates objects in a shelf. Since only lateral view is available, some objects are partially or even fully occluded by others, preventing perception modules from understanding the scene effectively. Moreover, the confined workspace can easily incur undesirable robot-object and object-object collisions, posing challenges to safety guarantees, which can be essential in handling vulnerable and fragile objects. One way to ensure safety is to plan conservative pick-and-place paths, which can be challenging as the action space is very limited. Beyond avoiding undesirable collisions, in-place manipulation of objects, where no extra buffer space is provided, introduces the additional challenge of identifying the right placement of objects in a confined workspace. To tackle partial observability, it is important to explore the environment, which involves, but not limited to object reconstruction, relocating objects to reveal other objects and reasoning the dependencies between them.

A series of efforts refer to the objective of locating and retrieving a hidden object as "Mechanical Search". Learning-based methods have been increasingly applied to this task \cite{huang2020mechanical,bejjani2021occlusion}. These methods, however, do not provide guarantees on safety and completeness. There are work \cite{dogar2014object,nam2021fast}, which provide some level of completeness but require extra buffers and assume a strong perception module, which can perfectly recognize objects with partial view. The most related work \cite{gupta2013interactive} proposes an adaptive search algorithm to explore the environment and retrieve a target object in a simplified setup without geometric analysis of occlusion space. 

Most existing work assume known object models and do not handle in-place relocation under occlusion. Completeness study is also missing for the object reconstruction task. Thus, the current work formulates and constructs a complete algorithm for object reconstruction in a confined space, where only in-place movements are allowed. The main contribution of this paper can be summarized as follows:
\begin{enumerate}
\item  A classification of problems in general object manipulation under occlusion.
\item A novel formalization for the task of reconstructing unknown objects.
\item An algorithmic framework for object exploration with in-place rearrangement under occlusion with an accompanying proof of completeness.
\item An instantiation of the above framework for monotone problems, which in experiments shows significant improvements against a random and a greedy baseline in terms of computation time and number of actions taken, with high success rate across experiments.
\end{enumerate}
